End behavior of Ramanujan's taxicab numbers

Generalized taxicab numbers are the smallest positive integers that are the sum of exactly $j$, positive $k$-th powers in exactly $m$ distinct ways. This paper is considers for which values of $m$ does a smallest such integer exist as $j$ gets large. There appear to be only two possible outcomes, leading to curious results like there is no positive integer that can be expressed as the sum of exactly $10$ positive squares in exactly $3$ ways. This paper resolves a number of conjectures found in the OEIS by considering generalized Taxicab numbers in the setting of the theory of partitions.

==> bibliography.tex <==
\begin{thebibliography}{10}

  \bibitem{Abramowitz}
  M.~Abramowitz, I.~A. Stegun, and R.~H. Romer.
  \newblock Handbook of mathematical functions with formulas, graphs, and
    mathematical tables, 1988.
  
  \bibitem{ahlgren}
  S.~Ahlgren and J.~Lovejoy.
  \newblock The arithmetic of partitions into distinct parts.
  \newblock {\em Mathematika}, 48(1-2):203–211, 2001.
  
  \bibitem{Andrews}
  G.~E. Andrews.
  \newblock {\em The theory of partitions}.
  \newblock Number~2. Cambridge University Press, 1998.
  
  \bibitem{Benfield}
  B.~Benfield, M.~Paul, and A.~Roy.
  \newblock Tur\`an inequalities for $k$-th power partition functions.
  \newblock {\em Journal of Mathematical Analysis and Applications},
    529(1):127678, 2024.
  
  \bibitem{Bernt}
  B.~C. Berndt.
  \newblock {\em Ramanujan’s Notebooks Part IV}.
  \newblock Springer New York, NY, 1994.
  
  \bibitem{Bernstein}
  D.~J. Bernstein.
  \newblock Enumerating solutions to p(a) + q(b) = r(c) + s(d).
  \newblock {\em Mathematics of Computation}, 70:389–394, 2001.
  
  \bibitem{Boyer}
  C.~Boyer.
  \newblock New upper bounds for taxicab and cabtaxi numbers.
  \newblock {\em Journal of Integer Sequences}, 11(08.1.6), 2008.
  
  \bibitem{Claude}
  C.~S. Calude, E.~Calude, and M.~J. Dinneen.
  \newblock What is the value of taxicab(6)?
  \newblock {\em Journal of Universal Computer Science}, 9:1196--1203, 2003.
  
  \bibitem{Descartes}
  R.~Descartes.
  \newblock Oeuvres.
  \newblock letters to Mersenne from July 27 and Aug 23, 1638.
  \newblock Paris.
  
  \bibitem{Dinitz}
  J.~H. Dinitz, R.~Games, and R.~Roth.
  \newblock Seeds for generalized taxicab numbers.
  \newblock {\em Journal of Integer Sequences}, 22:19.3.3, 2019.
  
  \bibitem{Dubouis}
  E.~Dubouis.
  \newblock Solution of a problem of {J}. {T}annery.
  \newblock {\em Interm\'ediaire Math}, 18:55--56, 1911.
  
  \bibitem{Ekl}
  R.~L. Ekl.
  \newblock New results in equal sums of like powers.
  \newblock {\em Mathematics of Computation}, 67(223):1309–1315, July 1998.
  
  \bibitem{Escott}
  E.~B. Escott.
  \newblock R\'eponse 1882, trouver quatre nombres tels que la somme de deux
    quel-conques d’entre eux soit un cube.
  \newblock {\em L’Interm\'ediaire des Math\'ematiciens}, (9):16–17, 1902.
  
  \bibitem{Euler}
  L.~Euler.
  \newblock Resolutio formulae {D}iophanteae ab(maa+nbb) = cd(mcc+ndd) per
    numeros rationales.
  \newblock {\em Nova Acta Academiae Scientiarum Imperialis Petropolitanae},
    1802.
  
  \bibitem{[Gafni]}
  A.~Gafni.
  \newblock Power partitions.
  \newblock {\em Journal of Number Theory}, 163:19--42, 2016.
  
  \bibitem{Grosswald}
  E.~Grosswald.
  \newblock {\em Representations of Integers as Sums of Squares}.
  \newblock Springer New York, NY, 1985.
  
  \bibitem{Hardy}
  G.~H. Hardy.
  \newblock {\em Ramanujan}.
  \newblock Cambridge Univ. Press, 1940.
  
  \bibitem{Hollerbach}
  U.~Hollerbach.
  \newblock ``{T}he sixth taxicab number is 24153319581254312065344.", Mar. 8,
    2008.
  
  \bibitem{kim}
  D.~Kim and A.~J. Yee.
  \newblock A note on partitions into distinct parts and odd parts.
  \newblock {\em The Ramanujan Journal}, 3:227--231, 1999.
  
  \bibitem{Lagrange}
  J.~L. Lagrange.
  \newblock D\'emonstration d'un or\'eme d'arithm\'etique.
  \newblock {\em Nouveaux m\'emoires de l'Acad\'emie royale des sciences et
    belles-lettres de Berlin, Anne\'e}, page 123–133, 1770.
  
  \bibitem{Leech}
  J.~Leech.
  \newblock Some solutions of {D}iophantine equations.
  \newblock In {\em Mathematical Proceedings of the Cambridge Philosophical
    Society}, volume~53, pages 778--780. Cambridge University Press, 1957.
  
  \bibitem{Frenicle}
  P.~Mancosu.
  \newblock Correspondence of {J}ohn {W}allis (1616-1703). vol. {I} (1641-1659),
    2006.
  
  \bibitem{Moore}
  D.~Moore.
  \newblock Cabtaxi(9).
  \newblock NMBRTHRY Archives e-mail, February 5, 2005.
  
  \bibitem{Pall}
  G.~Pall.
  \newblock On sums of squares.
  \newblock {\em The American Mathematical Monthly}, 40(1):10--18, 1933.
  
  \bibitem{Rathbun}
  R.~L. Rathbun.
  \newblock Sixth taxicab number?
  \newblock NMBRTHRY Archives e-mail, July 16, 2002.
  
  \bibitem{Dardis}
  E.~Rosenstiel, J.A. Dardis, and C.R. Rosenstiel.
  \newblock The four least solutions in distinct positive integers of the
    {D}iophantine equation s= x3+ y3= z3+ w3= u3+ v3= m3+ n3.
  \newblock {\em The Institute of Mathematics and its Applications Bulletin},
    27:155--157, 1991.
  
  \bibitem{A025416}
  N.~J.~A. Sloane and The OEIS~Foundation Inc.
  \newblock The on-line encyclopedia of integer sequences {A}025416.
  \newblock http://oeis.org/A025416, 2012.
  
  \bibitem{OEIS}
  N.~J.~A. Sloane and The OEIS~Foundation Inc.
  \newblock The on-line encyclopedia of integer sequences.
  \newblock http://oeis.org/, 2023.
  
  \bibitem{A080673}
  N.~J.~A. Sloane and The OEIS~Foundation Inc.
  \newblock The on-line encyclopedia of integer sequences {A}080673.
  \newblock http://oeis.org/A080673, 2023.
  
  \bibitem{A295702}
  N.~J.~A. Sloane and The OEIS~Foundation Inc.
  \newblock The on-line encyclopedia of integer sequences {A}295702.
  \newblock http://oeis.org/A295702, 2023.
  
  \bibitem{A295795}
  N.~J.~A. Sloane and The OEIS~Foundation Inc.
  \newblock The on-line encyclopedia of integer sequences {A}295795.
  \newblock http://oeis.org/A295795, 2023.
  
  \bibitem{[Vaughan]}
  R.~C. Vaughan.
  \newblock Squares: additive questions and partitions.
  \newblock {\em International Journal of Number Theory}, 11(05):1367--1409,
    2015.
  
  \bibitem{Vi`ete}
  D.~T. Whiteside.
  \newblock Fran{\c{c}}ois vi{\`e}te, the analytic art. nine studies in algebra,
    geometry and trigonometry from the ‘opus restitutae mathematics analyseos,
    seu algebra nova’.
  \newblock {\em The British Journal for the History of Science}, 18(1):98--100,
    1985.
  
  \bibitem{Wilson}
  D.~W. Wilson.
  \newblock The fifth taxicab number is 48988659276962496.
  \newblock {\em J. Integer Seq}, 2(99.1.9), 1999.
  
  \bibitem{[Wright]}
  E.~M. Wright.
  \newblock Asymptotic partition formulae. {III}. {Partitions} into {{\(k\)}}-th
    powers.
  \newblock {\em Acta Mathematica}, 63(1):143--191, 1934.
  
  \end{thebibliography}
  
